Sparse groups need not be semisparse

In 1999 Michael Hartley showed that any abstract polytope can be constructed as a double coset poset, by means of a C-group $\C$ and a subgroup $N \leq \C$. Subgroups $N \leq \C$ that give rise to abstract polytopes through such construction are called {\em sparse}. If, further, the stabilizer of a base flag of the poset is precisely $N$, then $N$ is said to be {\em semisparse}. In \cite[Conjecture 5.2]{hartley1999more} Hartley conjectures that sparse groups are always semisparse. In this paper, we show that this conjecture is in fact false: there exist sparse groups that are not semisparse. In particular, we show that such groups are always obtained from non-faithful maniplexes that give rise to polytopes. Using this, we show that Hartely's conjecture holds for rank 3, but we construct examples to disprove the conjecture for all ranks $n\geq 4$.

==> 2-face.tex <==
\newrgbcolor{ffdxqq}{1. 0.8431372549019608 0.}
\newrgbcolor{color1}{0. 0.8431372549019608 0.}
%\newrgbcolor{color1}{0. 104. 0.}
\psset{xunit=1.0cm,yunit=1.0cm,algebraic=true,dimen=middle,dotstyle=o,dotsize=4pt 0,linewidth=1.6pt,arrowsize=3pt 2,arrowinset=0.25}
\begin{pspicture*}(0.06477960908041465,-0.5548892341390115)(9.23899751999578,4.172381383846519)
\psline[linewidth=1.pt,linecolor=ffdxqq](1.,3.)(1.,2.)
\psline[linewidth=1.pt,linecolor=ffdxqq](2.,3.)(2.,2.)
\psline[linewidth=1.pt,linecolor=ffdxqq](3.,3.)(3.,2.)
\psline[linewidth=3.pt,linecolor=ffdxqq](4.,3.)(4.,2.)
\psline[linewidth=1.pt,linecolor=ffdxqq](5.,3.)(5.,2.)
\psline[linewidth=1.pt,linecolor=ffdxqq](6.,3.)(6.,2.)
\psline[linewidth=1.pt,linecolor=ffdxqq](7.,3.)(7.,2.)
\psline[linewidth=1.pt,linecolor=ffdxqq](8.,3.)(8.,2.)
\psline[linewidth=1.pt,linecolor=color1](1.,3.)(2.,3.)
\psline[linewidth=1.pt,linecolor=color1](3.,3.)(4.,3.)
\psline[linewidth=1.pt,linecolor=color1](5.,3.)(6.,3.)
\psline[linewidth=1.pt,linecolor=color1](7.,3.)(8.,3.)
\psline[linewidth=1.pt,linecolor=color1](8.,2.)(7.,2.)
\psline[linewidth=1.pt,linecolor=color1](6.,2.)(5.,2.)
\psline[linewidth=3.pt,linecolor=color1](4.,2.)(3.,2.)
\psline[linewidth=1.pt,linecolor=color1](2.,2.)(1.,2.)
\psline[linewidth=1.pt,linecolor=cyan](2.,3.)(3.,3.)
\psline[linewidth=1.pt,linecolor=cyan](3.,2.)(2.,2.)
\psline[linewidth=3.pt,linecolor=cyan](4.,3.)(5.,3.)
\psline[linewidth=1.pt,linecolor=cyan](5.,2.)(4.,2.)
\psline[linewidth=1.pt,linecolor=cyan](6.,2.)(7.,2.)
\psline[linewidth=1.pt,linecolor=cyan](7.,3.)(6.,3.)
\parametricplot[linewidth=1.pt,linecolor=cyan]{1.0523787347961537}{2.0892139187936394}{1.*7.063482735977398*cos(t)+0.*7.063482735977398*sin(t)+4.5|0.*7.063482735977398*cos(t)+1.*7.063482735977398*sin(t)+-3.135371900826449}
\parametricplot[linewidth=1.pt,linecolor=cyan]{4.193971388385947}{5.2308065723834325}{1.*7.063482735977398*cos(t)+0.*7.063482735977398*sin(t)+4.5|0.*7.063482735977398*cos(t)+1.*7.063482735977398*sin(t)+8.13537190082645}
\psline[linewidth=1.5pt,linecolor=cyan](0.95672,0.)(1.74672,0.)
\psline[linewidth=1.5pt,linecolor=color1](2.54946,0.)(3.33946,0.)
\psline[linewidth=1.5pt,linecolor=ffdxqq](4.20592,0.)(4.99592,0.)
\begin{scriptsize}
\psdots[dotstyle=*](1.,3.)
\psdots[dotstyle=*](2.,3.)
\psdots[dotstyle=*](2.,2.)
\psdots[dotstyle=*](1.,2.)
\psdots[dotstyle=*](3.,3.)
\psdots[dotstyle=*](3.,2.)
\psdots[dotsize=6pt 0,dotstyle=*](4.,3.)
\rput[bl](4.05301600646445,3.1785077768306933){\large{$x$}}
\psdots[dotstyle=*](4.,2.)
\psdots[dotstyle=*](5.,3.)
\psdots[dotstyle=*](5.,2.)
\psdots[dotstyle=*](6.,3.)
\psdots[dotstyle=*](7.,3.)
\psdots[dotstyle=*](8.,3.)
\psdots[dotstyle=*](8.,2.)
\psdots[dotstyle=*](7.,2.)
\psdots[dotstyle=*](6.,2.)
\rput[bl](1.2497827559069827,-0.25){{$0$}}
\rput[bl](2.82978695167574,-0.25){{$1$}}
\rput[bl](4.486242963368792,-0.25){{$3$}}
\end{scriptsize}
\end{pspicture*}

==> Construction.tex <==
We have seen that in order to find a group that is sparse but not semisparse we need to have a unfaithful maniplex that is polytopal.
In this section we construct such maniplex for $n=4$. 
\Cref{sec:extensions} will then use this maniplex to construct unfaithful maniplexes of rank $n>4$ that are polytopal.



\subsection{Double covers from voltage assignments}\label{sec:construction}

Let $\Gamma$ be a graph with edge-set $E$. A {\em $\ZZ_2$-voltage assignment} is a function $\zeta\colon E \to \ZZ_2$. The {\em double cover} of $\Gamma$ relative to $\zeta$, denoted $\Cov(\Gamma,\zeta)$, is the graph with vertex-set $V \times \ZZ_2$ and where two vertices $(x,i)$ and $(y,j)$ are adjacent if and only if $e:=\{x,y\}$ is an edge of $\Gamma$ and $j = i + \zeta(e)$.

Note that the mapping $\pi\colon \Cov(\Gamma,\zeta) \to \Gamma$ sending every vertex $(x,i)$ to $x$ is a quotient projection and thus $\Gamma$ is a quotient of $\Cov(\Gamma,\zeta)$. When $\Gamma$ is a rank $n$ maniplex, we can give a proper colouring to $\Cov(\Gamma,\zeta)$ by colouring every edge $e$ with the same colour as $\pi(e)$. Note that this is not enough to guarantee that $\Cov(\Gamma,\zeta)$ is an $n$-maniplex.

\begin{lemma}
\label{lem:voltcon}
Let $\Gamma$ be a connected graph, let $\zeta$ be a $\ZZ_2$-voltage assignment and let $\Gamma'$ be a connected subgraph of $\Gamma$. If the set of edges of $\Gamma'$ with non-trivial voltage is not a cut-set of $\Gamma'$, then $\pi^{-1}(\Gamma')$ is connected. %In particular, if all the edges of $\Gamma'$ have trivial voltage, then $\pi^{-1}(\Gamma')$ is connected. \isa{A\~nad\'i un caso particular}
\end{lemma}

\begin{lemma}
\label{lem:voltmani}
Let $\Gamma$ be a connected graph and let $\zeta$ be a $\ZZ_2$-voltage assignment. Then $\Cov(\Gamma,\zeta)$ is a maniplex if and only if the following hold:
\begin{enumerate}
\item the set of edges of $\Gamma$ with non-trivial voltage is not a cut-set;
\item every $4$-cycle of $\Gamma$ of alternating colours $i$ and $j$, with $|i-j|>1$, has an even number of edges with non-trivial voltage.
\end{enumerate}
\end{lemma}


\subsection{A unfaithful polytopal $4$-maniplex}


The goal of this construction is to obtain a unfaithful $4$-maniplex whose poset is an abstract polytope. 
To do so, we shall start with a faithful $4$-maniplex $\B$ that is polytopal and reflexible.%\isa{Cambi\'e la redacci\'on porque la notaci\'on $\{\{4,3\}_3,\{3,4\}_3\}$ es muy de politopos y no creo que se haya usado para maniplexes. Entonces lo escrib\'i de forma que $\B$ sea la gr\'afica de banderas del politopo. A\~nad\'i tambi\'en informaci\'on del politopo }
%The basis for the construction is the regular polytopal $4$-maniplex $\{\{4,3\}_3,\{3,4\}_3\}$, which we will call $\B$.
Then, we shall construct a double cover $\B^*$ of $\B$ such that for all $i \in \{0,1,2,3\}$ and every $i$-face $F$ of $\B$, the lift $\pi^{-1}(F)$ is connected, and thus an $i$-face of $\B^*$.
This will imply that there is a bijection between the $i$-faces of $\B$ and the $i$-faces of $\B^*$ that will preserve the order, implying that $\B^*$ and $\B$ have isomorphic posets.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.85\textwidth]{posetB.png}
\caption{The self-dual regular $4$-polytope $\po$}
\label{fig:pos}
\end{center}
\end{figure}

Let $\po$ be the regular $4$-polytope $\{\{4,3\}_3,\{3,4\}_3\}$. This polytope is denoted by $\{4,3,4\}^*96$ in \cite{hartley2006atlas}. It is the universal polytope whose facets are hemi-cubes $\{4,3\}_3$, and whose vertex-figures are hemi-octahedra $\{3,4\}_3$, and has a total of $96$ flags. 
It has $4$ vertices, $6$ edges, $6$ polygons (or $2$-faces) and $4$ facets, from which we can see that it is a flat polytope (that is, every vertex belongs to every facet).%\isa{quiz\'a es buena idea poner aqu\'i un dibujo del diagrama de Hasse de $\po$ sin marcar ninguna bandera, solo para que est\'e de referencia} \micael{la verdad no se si ayude mucho a entender quiene es $\po$}
%\isa{No lo pensaba tanto para entender $\po$ en s\'i, sino los conjuntos de banderas que se colorean}
%
\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.85\textwidth]{posets2.png}
\caption{The distinguished sets of flags $X^0$, $X$ and $X^3$ (the minimal and maximal faces are not shown)}
\label{fig:pos}
\end{center}
\end{figure}
%
Let $\B$ be the flag graph of $\po$. Then $\B$ is a faithful polytopal $4$-maniplex, and the flags of $\po$ are in one-to-one correspondence with the vertices of $\B$.
To construct the double cover of $\B^*$, we need to define a $\ZZ_2$-voltage assignment for the edges of $\B$.
To do so, we will use the Hasse diagram of $\po$ to define some sets of vertices and edges of $\B$.
% \begin{figure}[h!]
% \begin{center}
% \includegraphics[width=0.85\textwidth]{posets2.png}
% \caption{Three copies of $\po$ with the distinguished sets of flags $X^0$, $X$ and $X^3$.}
% \label{fig:pos}
% \end{center}
% \end{figure}
%
\isa{Creo que ser\'ia buena idea poner los diagramas de $X^{02}$ y $X^{31}$ para que sea f\'acil de seguir el lema de abajo}
Let $X$ be the set of flags of $\B$ corresponding to the maximal chains of $\po$ drawn in bold black edges, in the centre of Figure \ref{fig:pos}. 
For $i \in [4]$, let $X^i = \{x^i \mid x \in X \}$. The sets $X^0$ and $X^3$ are depicted (as chains on a poset) in the left-hand and right-hand side of Figure \ref{fig:pos}, respectively. We have chosen the flags of $X$ so that $X$ has certain desirable properties. In particular if $F$ is an $i$-face of $\B$ (that is, a connected component of $\B_{\hat{i}}$%\isa{a\~nad\'i esta frase, pero en realidad no s\'e si m\'as bien hay que escribirlo en t\'erminos de $\po$, porque lo que se dice lo ves en los dibujos de $\po$, m\'as que en la gr\'afica $\B$. Revisandolo en el dibujo y leyendo contiene en vez de est\'a contenido, mi cabeza se hace bolas...}), \micael{Veo tu punto. Quiza hasta valaga la pena tener dos versiones. Primero decirlo en $\po$ y luego la version "traducida"} 
then the following hold:
%
\begin{enumerate}
\item[(A.1)] If $i \in \{1,2\}$, then $F$ contains exactly one flag $x \in X$;
\item[(A.2)] If $i \in \{0,3\}$, then $F$ contains either exactly one or exactly two flags in $X$;
\item[(A.3)] If $i \in \{0,3\}$ and $F$ contains two flags in $X$, then these flags lie on different $j$-faces for all $j \neq i$. Moreover, $F$ contains exactly one flag in $X^i$;
\item[(A.4)] If $i \in \{0,3\}$ and $F$ contains only one flag in $X$, then it contains exactly two flags in $X^i$.
\end{enumerate}

To define a voltage assignment for $\B$, we will need to define a set of links\isa{En la parte de dobles cubiertas se dice que los voltajes van a los darts, hay que ponerlo igual en todas partes } $E_X$, to carry non-trivial voltages. First, for each $x \in X$, let $E_x$ be the set of links $\{xx^0,x^0x^{02},xx^3,x^3x^{31}\}$. Note that the links of $E_x$ are the links of a $1302$-path starting at $x^{31}$ and ending in $x^{02}$ (see Figure \ref{fig:voltaje}). Let $E_X = \bigcup_{x \in X} E_x$. 
%\isa{Creo que es buena idea cambiar el rojo de aqu\'i, porque eran las de $X$ y aqu\'i son las $2$-adjacentes}


\begin{figure}[H]
\begin{center}
\includegraphics[width=0.35\textwidth]{voltaje.png}
\caption{Part of the intersection of a $1$- with a $2$-face. A set $E_x$ shown in thick edges.}
\label{fig:voltaje}
\end{center}
\end{figure}



\begin{lemma}
Let $F$ be an $i$-face of $\B$. If $i \in \{1,2\}$ then all the following hold:
\begin{enumerate}
\item[(B.1)] If $uv$ is an $i$-link in $E_X$, then either $u \in X^{i+2}$ or $v \in X^{i+2}$, where addition is taken modulo $4$;
\item[(B.2)] If $uv$ is an $i$-link in $E_X$, then $\{u,v\} \cap X = \emptyset$.
\item[(B.3)] There is exactly one $j$-link in $E_X \cap F$ for each $j \in \{0,1,2,3\}\setminus\{i\}$.
\end{enumerate}

Moreover if $i \in \{0,3\}$ then one of the following holds: 
\begin{enumerate}
\item[(B.4)] $F$ contains exactly two $j$-links in $E_X$ for each $j \in \{i+1,i-1\}$ and one $(i+2)$-link in $E_X$;
\item[(B.4)'] $F$ contains exactly one $j$-link in $E_X$ for each $j \in \{i+1,i-1\}$ and two $(i+2)$-links in $E_X$;
\end{enumerate}
\end{lemma}

\begin{proof}
Item (B.1) and (B.2) follow from the definition of $E_X$.

%Item (B.3) follows from (A.1). 
For item (B.3), let us assume that $i=2$ (a similar argument applies for $i=1$).
First, let $x$ be the flag in $x\in F\cap X$; it exists and it is unique by (A.1). 
Since all the $0$- and $3$-links of $E_X$ have one vertex in $X$, then the only $0$- and $3$-links in $E_X\cap F$ are precisely $xx^0$ and $xx^3$.
Now, the $1$-links of $E_X$ are all of the form $y^3y^{31}$, for some $y\in X$. 
Note that $y$ and $y^3$ are in the same $2$-face, so if $y^3y^{31}$ is a $1$-link in $E_X\cap F$, then $y\in X\cap F$, and therefore again by (A.1) $y=x$, implying there is only $1$-link in $E_X\cap F$.


Finally, observe that if $i \in \{0,3\}$ then one of the (A.3) and (A.4) hold for $F$. 
It is straightforward to see that if (A.3) holds, then so does (B.4).
Similarly, if (A.4) holds, then (B,4)' does as well.
\end{proof}

\begin{figure}[h]
    \centering
    \input{2-face}
    \caption{A $2$-face of $\B$, with its intersection with $E_X$ shown in thick edges. }
    \label{fig:2-face}
\end{figure}

%\micael{Puse dos versiones de los dibujos. Poniendo las aristas en $E_X$ gorditas, medio se pierden entre tanta arista, entonces hice las aristas sin voltaje transparentes. La otra opcion es ponerlas punteadas (en esta version tambien cambie el acomodo de los vertices en X, pero son equivalentes), pero entonces quiza tengamos que ponerlas punteadas en todos los dibujos, para ser consistentes}


\begin{figure}[H]
\begin{center}
\includegraphics[width=1\textwidth]{4facetas.png}
\caption{The four facets of $\B$, with its intersection with $E_X$ shown in thick edges.}
\label{fig:voltaje}
\end{center}
\end{figure}

%\begin{figure}[H]
%\begin{center}
%\includegraphics[width=1\textwidth]{4facetas2.png}
%\caption{The four facets (laternative version)}
%\label{fig:voltaje}
%\end{center}
%\end{figure}

%\isa{me gustan m\'as gorditas, me cuesta trabajo encontrarlas cuando est\'an punteadas}
Now we are ready to define a $\ZZ_2$-voltage assignment $\zeta_X: \E(\B) \to \ZZ_2$. We let

\[
\zeta_X(e)=
 \begin{cases}
1 & \text{ if $e \in E_X$}   \\
0 & \text{ otherwise.}
\end{cases}
\]

Recall that a covering graph $\Cov(\M,\zeta)$ is connected if the edges with non-trivial voltage are not a cut-set, by Lemma \ref{lem:voltcon}
%and let $\overline{\B}$ denote the derived cover of $(\B,\zeta_X)$.

\begin{lemma}
\label{lem:12face}
If $F$ is an $i$-face of $\B$ with $i \in \{1,2\}$, then $\pi^{-1}(F)$ is a connected subgraph of $\Cov(\B,\zeta_X)$.
\end{lemma}

\begin{proof}
%\isa{hab\'ia una cosa en una frase de la prueba que no entend\'i. En cualquier caso pens\'e que es las 1- y 2- caras son en realidad muy sencillas, as\'i que puse el dibujo de una 2-cara para usarlo en el argumento, que se vuelve m\'as f\'acil de seguir. la frase que no entend\'i est\'a comentada, por si queremos regresar a ella}
By (B.3) $F$ contains exactly one $j$-link of $E_X$ for each $j \in \{0,1,2,3\}\setminus\{i\}$. 
As $F$ contains no $i$-links, those three links are the only links in $F \cap E_X$.
%Moreover, by (B.2) these\isa{which are ``these'' links? the $0$-link and the $3$-link in $F \cap E_X$ share the flag of $x$ that is contained in $F$} links do not share a common endpoint. 
%Therefore,
Let $F^-$ be the graph obtained by removing the links in $F\cap E_X$  from $F$.
Note that $F^-$ remains connected (see \Cref{fig:2-face} for the case $i=2$, the figure for $i=1$ is similar).
Since every link lying on $F^-$ has trivial voltage, by \Cref{lem:voltcon}  $\pi^{-1}(F)$ is connected. 
\end{proof}

\begin{lemma}
\label{lem:03face}
If $F$ is an $i$-face of $\B$, $i \in \{0,3\}$, then $\pi^{-1}(F)$ is a connected subgraph of $\Cov(\B,\zeta_X)$.
\end{lemma}

\begin{proof}
There are two cases to consider, depending on which of the conditions (B.4) and (B.4)' is satisfied by $F$. For the sake of simplicity, we may assume $i = 3$, and the case $i = 0$ will follow by duality.

First, suppose that $(B.4)$ holds (and thus also (A.3)). That is, there are exactly two flags $u,v \in F \cap X$. Furthermore, there are exactly five links in $F \cap E_X$: the $0$- and $2$-links incident to $u$ and $v$ and a single $1$-link.
%
Let $F'$ be the graph resulting from the deletion of the $0$- and $2$-links in $F \cap E_X$. Note that $F'$ can only be disconnected if $u$ and $v$ are the endpoints of a $1$-link. However, this cannot happen because then $u$ and $v$ would lie on the same $2$-face, contradicting (A.3). Now, the deletion of a $1$-link $e$ disconnects $F'$ only if one of $u$ or $v$ is an endpoint of $e$, but this cannot happen either since, by (B.2), no endpoint of $e$ is an element of $X$.
If follows that the graph obtained from $F$ after the deletion of the links in $F \cap E_X$ is connected. Therefore $\pi^{-1}(F)$ is connected by \Cref{lem:voltcon}. 

Now, suppose $(B.4')$ holds. Then $F \cap E_X$ consists of two $1$-links and one $j$-link for each $j \in \{0,2\}$. 
Moreover, the $0$- and $2$-links share a common endpoint, $u$, which is an element of $X^0$. %\isa{Los links de $E_X$ conectados a elementos de $X$ tiene colores $0$ y $3$. La bandera en la que se intersectan es $u^0$, no?}
Let $F'$ be the graph resulting from the deletion of the links in $F \cap E_X$ from $F$. Again, $F'$ can only be disconnected if $u$ is an endpoint of one of the $1$-links in $F \cap E_X$, but by the definition of $\zeta_X$, no flag of $\B$ is incident to three links in $E_X$.
%this would contradict $(B.2)$\isa{como hay que cambiar $u$ por $u^0$ entonces (B.2) ya no aplica aqu\'i. (De hecho (B.2) te dice que $u$ no puede estar en un $2$-link de $E_X$)}. Then $F'$ is connected and therefore so is $\pi^{-1}(F)$.
\end{proof}


\begin{figure}[h!]
\label{fig:pos}
\begin{center}
\includegraphics[width=0.25\textwidth]{faceta.png}
\caption{A facet of $\po$, isomorphic to a hemicube, seen as a subgraph of $\B$.}
\end{center}
\end{figure}

\begin{lemma}
\label{lem:Bstarmani}
The covering graph $\B^*:=\Cov(\B,\zeta_X)$ is a maniplex.
\end{lemma}

\begin{proof}
We need to prove that $\B^*$ is connected and that every $ijij$-path is a cycle of length $4$ whenever $|i-j| >1$. Let us begin by proving that $\B^*$ is connected.
Recall that the flags of $\B^*$ are of the form $(u,r)$ where $u$ is a flag of $\B$ and $r \in \{0,1\}$. 

By Lemmas \ref{lem:12face} and \ref{lem:03face}, we see that if $(u,r)$ is a flag of $\B^*$, then $\B^*_{\bar{i}}((u,r)) = \pi^{-1}(\B_{\bar{i}}(u))$. Moreover, two subgraphs $\B^*_{\bar{i}}((u,r))$ and $\B^*_{\bar{j}}((u',r'))$ have non-trivial intersection if and only if the corresponding projections $\B_{\bar{i}}(u)$ and $\B_{\bar{j}}(u')$ have non-trivial intersection. The connectedness of $\B^*$ then follows from the fact that $\B^*_{\bar{i}}((u,r)) = \pi^{-1}(\B_{\bar{i}}(u))$ for all $(u,r) \in \B*$ and $i\in\{0,1,2,3\}$ and that $\B$ is connected.

Now, let $C$ be an $ijij$-path in $\B$ with $|i-j|>1$.  Then, there are only two options for the voltages of the links in $C$: either all links in $C$ have trivial voltage, or two consecutive links (and only these two) have trivial voltage. In either case, the number of edge with non-trivial voltage is even and by Lemma \ref{lem:voltmani}, we conclude that $\B^*$ is a maniplex.
\end{proof}

Lemmas \ref{lem:12face}, \ref{lem:03face} and \ref{lem:Bstarmani} combined give us:

\begin{proposition}\label{prop:sameposet}
The covering graph $\Cov(\B,\zeta_X)$ is a $4$-maniplex with the same poset as $\B$.
\end{proposition}

We have therefore showed that $\B^*=\Cov(\B,\zeta_X)$ is a connected graph (\Cref{lem:Bstarmani}) that has vertex set $\B \times \mathbb{Z}_2$. That is, $\B*$ has twice as many vertices as $\B$.
\Cref{prop:sameposet} implies that $\Pos(\B^*)=\Pos(\B)$, implying that the number of flags of $\Pos(\B^*)$ is half the numer of vertices of $\B^*$ and therefore $\B^*$ is unfaithful.
Moreover, $\Pos(\B^*)=\Pos(\B)=\po$, which means that $\B^*$ is a polytopal maniplex.
We have therefore established the following results.

\begin{proposition}
    $\B^*$ is an unfaithful polytopal $4$-maniplex.
\end{proposition}

The above theorem and \Cref{unfaithfulpolytopal} imply that:

\begin{theorem}
    In rank $4$ there exists at least one sparse group that is not semisparse.
\end{theorem}


==> Maniplexes-and-semisparse.tex <==
\section{Maniplexes and double coset construction}


